PEGRL: Improving Machine Translation by Post-Editing Guided Reinforcement Learning

Reinforcement learning (RL) has shown strong promise for LLM-based machine translation, with recent methods such as GRPO demonstrating notable gains; nevertheless, translation-oriented RL remains challenged by noisy learning signals arising from Monte Carlo return estimation, as well as a large trajectory space that favors global exploration over fine-grained local optimization. We introduce \textbf{PEGRL}, a \textit{two-stage} RL framework that uses post-editing as an auxiliary task to stabilize training and guide overall optimization. At each iteration, translation outputs are sampled to construct post-editing inputs, allowing return estimation in the post-editing stage to benefit from conditioning on the current translation behavior, while jointly supporting both global exploration and fine-grained local optimization. A task-specific weighting scheme further balances the contributions of translation and post-editing objectives, yielding a biased yet more sample-efficient estimator. Experiments on English$\to$Finnish, English$\to$Turkish, and English$\leftrightarrow$Chinese show consistent gains over RL baselines, and for English$\to$Turkish, performance on COMET-KIWI is comparable to advanced LLM-based systems (DeepSeek-V3.2). Our code and a set of representative pretrained models are publicly available at \url{https://github.com/NJUNLP/peg-rl} and \url{https://huggingface.co/collections/DGME/pegrl}

==> fig/role_analysis.tex <==
\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{assets/MT_role_kiwi.pdf}
        \centering
    \end{minipage}
    % 第二张图
    \hfill
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{assets/MT_role_xcomet.pdf}
        \centering
    \end{minipage}
\caption{Evaluation results on WMT24 EN$\rightarrow$TR, reported every 20 training steps, comparing Ours-8B and MT-R1-Zero-8B. \emph{Ours w/o PE} denotes the draft translations produced by our first-stage model without post-editing.}

    \label{fig:role-ablation}
\end{figure}


==> fig/rollout.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{assets/rollout.pdf}
  \caption{Overview of the proposed rollout stage.}
  \label{fig:rollout}
\end{figure}

==> table/sentence_num.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
Setting & $\text{AvgU@64}$ & \text{PassU@64} \\
\midrule
EN $\to$ FI(MT) & 0.9352 & 0.6550 \\
EN $\to$ FI(PE) & 0.3417 & 0.0040 \\
EN $\to$ TR(MT) & 0.9042 & 0.5770 \\
EN $\to$ TR(PE) & 0.4407 & 0.0250 \\
\bottomrule
\end{tabular}
\caption{Quantitative analysis of output diversity for translation (MT) and post-editing (PE) on 1K sentences for En$\rightarrow$Fi and En$\rightarrow$Tr. For each input, we roll out 64 trajectories using Qwen3-4B. \textbf{AvgU@64} denotes the average number of unique outputs among the 64 samples, while \textbf{PassU@64} measures the fraction of inputs whose 64 rollouts are all distinct. As shown, post-editing exhibits substantially lower sampling diversity than translation.}

\label{tab:sampling_space}
\end{table}

